Analog Beamforming Codebooks for Wideband Full-Duplex Millimeter-Wave Systems

In full-duplex millimeter-wave (mmWave) systems, the effects of beam squint and the frequency-selectivity of self-interference exacerbate over wide bandwidths. This complicates the use of beamforming to cancel self-interference when communicating over bandwidths on the order of gigahertz. In this work, we present the first analog beamforming codebooks tailored to wideband full-duplex mmWave systems, designed to both combat beam squint and cancel frequency-selective self-interference. Our proposed design constructs such codebooks by minimizing self-interference across the entire band of interest while constraining the coverage provided by these codebooks across that same band. Simulation results using computational electromagnetics to model self-interference suggest that a full-duplex 60 GHz system with our design enjoys lower self-interference and delivers better coverage across bandwidths as wide as 6 GHz, when compared to similar codebook designs that ignore beam squint and/or frequency-selectivity. This allows our design to sustain higher SINRs and spectral efficiencies across wide bandwidths, unlocking the potentials of wideband full-duplex mmWave systems.

==> sec-formulation.tex <==
\section{Problem Formulation} \label{sec:problem-formulation}
In the original beamforming vector set, $\sF$ and $\sW$, there are so many candidates that it is impractical to determine beamforming vectors in the set. 
Hence, in this work, we aim to narrow down these sets to smaller subsets and make a codebook, which is denoted as $\overline{\sF} \subset \sF$ and $\overline{\sW} \subset \sW$. 
The size of the sets are referred to $\bars{\overline{\sF}} = \Mtx$ and $\bars{\overline{\sW}} = \Mrx$. 
To construct the codebook, we will firstly establish metrics.

%$\precbbar$

\subsection{Metrics of Codebook Design}
The signal-to-interference-plus-noise ratios (SINRs) at $k$th subcarrier can be described as
\begin{align}
    \sinrtx[k] = \frac{\snrtx[k]}{1 + \inrtx[k]}, \quad \quad \sinrtx[k] = \frac{\snrrx[k]}{1 + \inrrx[k]}.
\end{align}
each of which depends on the signal-to-noise ratio (SNR) and interference-to-noise ratio (INR).
With beamforming vectors $\vf$ and $\vw$, the SNR of the downlinks and uplinks are expressed as
\begin{align}
    &\snrtx[k] = \frac{\powertx^{\mathrm{BS}} \cdot \Gtx^2 \cdot \bars{\vfh_{\mathrm{tx}}^*[k] \vf}^2}{\Nt \cdot \powernoise^{\mathrm{UE}}} \label{SNR_tx},\\
    &\snrrx[k] = \frac{\powertx^{\mathrm{UE}} \cdot \Grx^2 \cdot \bars{\vfh_{\mathrm{rx}}^*[k] \vw}^2}{\normtwo{\vw}^2 \cdot \powernoise^{\mathrm{BS}}}. \label{SNR_rx}
\end{align}
where dividing by $\Nt$ in \eqref{SNR_tx} addresses power distribution within the transmit array, and by $\normtwo{\vw}^2$ in \eqref{SNR_rx} deals with noise aggregation at the receive array. 
Since these quantities are upper bounded as $\bars{\vfh_{\mathrm{tx}}^*[k] \vf}^2 \leq \Nt^2, \bars{\vfh_{\mathrm{rx}}^*[k] \vw}^2 \leq \Nr^2$ so that the bound of $\frac{1}{K}\sum_{k=1}^K\snrtx[k]$ and $\frac{1}{K}\sum_{k=1}^K\snrrx[k]$ is computed as
\begin{align}
    \overline{\mathsf{SNR}}_{\mathrm{tx}} = \frac{\Gtx^2 \cdot \Nt \cdot \powertx^{\mathrm{BS}}}{\powernoise^{\mathrm{UE}}} \geq \frac{1}{K}\sum_{k=1}^K\snrtx[k], \\
    \overline{\mathsf{SNR}}_{\mathrm{rx}} = \frac{\Grx^2 \cdot \Nr \cdot \powertx^{\mathrm{UE}}}{\powernoise^{\mathrm{BS}}} \geq \frac{1}{K}\sum_{k=1}^K\snrrx[k].
\end{align}
To capture how well a given beamforming vector aligns well with the channel, we will investigate the relative size of $\mathsf{SNR}$ comparing to $\overline{\mathsf{SNR}}$.
\begin{align}
    &\frac{\mathsf{SNR}_{\mathrm{tx}}[k]}{\overline{\mathsf{SNR}}_{\mathrm{tx}}} = \frac{\bars{\vfh^*_{\mathrm{tx}}[k] \vf}^2}{\Nt^2} \\
    &\frac{\mathsf{SNR}_{\mathrm{rx}}[k]}{\overline{\mathsf{SNR}}_{\mathrm{rx}}} = \frac{\bars{\vw^* \vfh_{\mathrm{rx}}[k]}^2}{\Nr \cdot \normtwo{\vw}^2}
\end{align}

Since the transmit beam $\vf$ and receive beam $\vw$ are intertwined with the self-interference channel, $\mfH[k]$, the uplink INR on subcarrier $k$ can be written as
\begin{align}
    \inrrx[k] = \frac{\powertx^{\mathrm{BS}} \cdot G^2 \cdot \bars{\vw^* \mfH[k] \vf}^2}{\Nt \cdot \normtwo{\vw}^2 \cdot \powernoise^{\mathrm{BS}}}.
\end{align}
When $\vf$ and $\vw$ are aligned in the direction that creates the strongest interaction, $\Nt^2\cdot\Nr^2 = \max\bars{\vw^*\mfH[k]\vf}^2$, the maximum $\inrrx$, $\overline{\inr}_{\mathrm{rx}}$ can be expressed as follows.
\begin{align}
    \overline{\inr}_{\mathrm{rx}} = \frac{G^2 \cdot \Nt \cdot \Nr \cdot \powertx^{\mathrm{BS}}}{\powernoise^{\mathrm{BS}}} \geq \frac{1}{K}\sum_{k=1}^K \inrrx[k].
\end{align}
Similarly, $\inrrx[k]$ can be represented as the relative format, $\frac{\mathsf{INR}_{\mathrm{rx}}[k]}{\overline{\mathsf{INR}}_{\mathrm{rx}}}$.
\begin{align}
    \frac{\mathsf{INR}_{\mathrm{rx}}[k]}{\overline{\mathsf{INR}}_{\mathrm{rx}}} = \frac{\bars{\vw^* \mfH[k] \vf}^2}{\Nt^2 \cdot \Nr \cdot \normtwo{\vw}^2}
\end{align}
Since user sides also operate in full-duplex mode, $\inrtx$, incurred by cross-link interference is calculated as follows.
\begin{align}
    \inrtx[k] = \frac{\powertx^{\mathrm{UE}}[k] \cdot G^2_{\mathrm{CL}} \cdot \bars{h_{\mathrm{CL}}[k]}^2}{\powernoise^{\mathrm{BS}}}
\end{align}
Note that there are no dependencies of $\vf$ and $\vw$ in the $\inrtx[k]$. 
Since the purpose of this work is to tactically steer direction of beams, we will not control the power of UE to decrease cross-link interference.

In this setting, the maximum achievable spectral of two links can be described as
\begin{align}
    \Rtx[k] = \log_2(1 + \sinrtx[k]), \quad \Rrx[k] = \log_2(1 + \sinrrx[k]),
\end{align}
and the channel capacities of two links are represented as $\Ctx[k] = \log_2(1 + \overline{\mathsf{SNR}}_{\mathrm{tx}}[k])$ and $\Crx[k] = \log_2(1 +\overline{\mathsf{SNR}}_{\mathrm{rx}}[k])$.
Let $\mathcal{A}_{\mathrm{tx}}$ be a transmit coverage region consisting $M_{\mathrm{tx}}$ transmit directions that the transmit codebook $\Bar{\mathcal{F}}$ takes responsibility to cater, and $\mathcal{A}_{\mathrm{rx}}$, a receive coverage region, is defined similarly to the transmit coverage region.
\begin{align}
    &\mathcal{A}_{\mathrm{tx}} = \{ \theta_{\mathrm{tx}}\idx{i} : i=1, \ldots, \Mtx \} \\
    &\mathcal{A}_{\mathrm{rx}} = \{ \theta_{\mathrm{rx}}\idx{j} : j=1, \ldots, \Mrx \}
\end{align}
where $\theta_{\mathrm{tx}}\idx{i}$ and $\theta_{\mathrm{rx}}\idx{j}$ are sets of azimuthal and elevational degree of each beams.
To make each $\Mtx$ beams of transmit array in $\Bar{\mathcal{F}}$ and $\Mrx$ beams of receive array in $\Bar{\mathcal{W}}$ indicate the directions of $\mathcal{A}_{\mathrm{tx}}$ and $\mathcal{A}_{\mathrm{rx}}$, we express beams as $\Bar{\mathcal{F}} = \{\vf_1, \ldots, \vf_{\Mtx} \}$ and $\Bar{\mathcal{W}} = \{\vw_1, \ldots, \vw_{\Mrx} \}$, where $\vf_i \in \Bar{\mathcal{F}}$ is in charge of transmitting toward $\theta_{\mathrm{tx}}\idx{i}$ and $\vw_j \in \Bar{\mathcal{W}}$ handles the reception of data from the direction, $\theta_{\mathrm{rx}}\idx{j}$. 
Under this notation, we construct the transmit codebook matrix $\mF$ by arranging the transmit beams $\vf_i$ in a stacked format, and codebook matrix $\mW$ is built in the same manner.
\begin{align}
    \mF &= [\vf_1 \quad \vf_2 \quad \cdots \quad \vf_{\Mtx}] \in \setmatrixcomplex{\Nt}{\Mtx} \\
    \mW &= [\vw_1 \quad \vw_2 \quad \cdots \quad \vw_{\Mrx}] \in \setmatrixcomplex{\Nr}{\Mrx}
\end{align}
The gain of the transmit beamforming vector, $\vf_i$ toward the direction $\thetatx^{(i)}$ at the $k$-th subcarrier is denoted as $\gtx^2(\thetatx^{(i)},k)$ and the gain of the receive beamforming vector, $\vw_j$ in the direction $\thetarx^{(j)}$ at the $k$-th subcarrier is expressed as $\grx^2(\thetarx^{(j)},k)$. 
They can be computed as follows:
\begin{align}
    &\gtx^2(\thetatx^{(i)}, k) = \bars{\vfatx^*(\thetatx^{(i)}, k) \vf_i}^2 \leq \Nt^2,  \ \forall \  k, \\
    &\grx^2(\thetarx^{(j)}, k) = \bars{\vfarx^*(\thetarx^{(j)}, k) \vw_i}^2 \leq \Nr^2,  \ \forall \  k.
\end{align}
The product $\vw_j^* \mfH[k] \vf_i$ captures the interaction between the i-th transmit beam $\vf_i$ and the j-th receive beam $\vw_j$ at the $k$-th carrier frequency and this concept can be generalized to include all transmit-receive beam combinations as $\mW^* \mfH[k] \mF \in \setmatrixcomplex{\Mrx}{\Mtx}$. 
In this work, we aim to minimize the holistic average interference over the all directions and frequencies of the subcarrier, which can be written as
\begin{align}
    \inrrx^{\mathrm{avg}} &= \frac{1}{K \cdot \Mtx \cdot \Mrx} \cdot \sum_{k=1}^K \sum_{i=1}^{\Mtx} \sum_{j=1}^{\Mrx} \frac{\powertx^{\mathrm{BS}} \cdot G^2 \cdot \bars{\vw_j^* \mfH[k] \vf_i}^2}{\Nt \cdot \normtwo{\vw_j}^2 \cdot \powernoise^{\mathrm{BS}}} \\
    &\approx \frac{G^2 \cdot \powertx^{\mathrm{BS}}}{\Nt \cdot \Nr \cdot K \cdot \powernoise^{\mathrm{BS}} } \cdot \sum_{k=1}^K \frac{\normfro{\mW^* \mfH[k] \mF}^2}{\Mtx \cdot \Mrx} \label{inrrxavg}
\end{align}
where $\normtwo{\vw_j}^2 \approx \Nr$ for all $j$. 
This approximation is satisfied when the gain of receive codebook is guaranteed.
Since all of the terms except for $\mW$ and $\mF$ are constant, the interference could be mitigated when $\sum_{k=1}^K \normfro{\mW^* \mfH[k] \mF}^2$ is minimized by designing $\mF$ and $\mW$. 
The trivial solution to minimize the $\inrrx^{\mathrm{avg}}$ without proper constraints is designing the beamforming codebook for $\mW$ to be zero, which makes the beamforming gain be vanished. Therefore, we force this system to maintain an adequate gain of the codebook while minimizing $\inrrx^{\mathrm{avg}}$. 
%The system should guarantee the small gap between the maximum gain in the transmit part and receive part over $\mathcal{A}_{\mathrm{tx}}$ and $\mathcal{A}_{\mathrm{rx}}$, respectively. 
In other words, difference between $\Nt$ and $\gtx(\thetatx^{(i)})$ and distinction between $\Nr$ and $\grx(\thetatx^{(j)})$ should be less than $\sigmatx^2 \geq 0$ and $\sigmatx^2 \geq 0$, the maximum tolerance of gain over all directions and frequencies. Thus, we can express these allowances as 
\begin{align}
    \frac{1}{\Mtx} \cdot \sum_{i=1}^{\Mtx} \frac{\bars{\Nt - \gtx(\thetatx^{(i)}, k)}^2}{\Nt^2} \leq \sigmatx^2  \ \forall \  k, \label{gain_tx_var}\\
    \frac{1}{\Mrx} \cdot \sum_{j=1}^{\Mrx} \frac{\bars{\Nr - \grx(\thetarx^{(j)}, k)}^2}{\Nr^2} \leq \sigmarx^2  \ \forall \  k. \label{gain_rx_var}
\end{align}
In this context, $\sigmatx^2$ and $\sigmarx^2$ are parameters set by system designers. 
By increasing these parameters, the system gains more flexibility in decreasing $\inrrx$, but this may lead to reduced gain due to increased variability in beamforming gain over the service areas.

The collection of transmit array response evaluated at the directions specified in $\mathcal{A}_{\mathrm{tx}}$ is represented by $\mAtx[k] \in \setmatrixcomplex{\Nt}{\Mtx}$, and $\mArx[k] \in \setmatrixcomplex{\Nr}{\Mrx}$ is defined analogously.
\begin{align}
    \mAtx[k] = \big[ \vatx(\thetatx^{(1)}, f_k) \ \ldots \ \vatx(\thetatx^{(\Mtx)},f_k) \big] \\
    \mArx[k] = \big[ \varx(\thetarx^{(1)}, f_k) \ \ldots \ \varx(\thetarx^{(\Mrx)},f_k) \big]
\end{align}
With these matrices, the \eqref{gain_tx_var} and \eqref{gain_rx_var} can be reformulated as follows.
\begin{align}
    \normtwo{\Nt \cdot \vone - \diag{\mAtx\ctrans[k]\mF}}^2 \leq \sigma_{\mathrm{tx}}^2 \cdot \Nt^2 \cdot \Mtx \ \forall \  k \\
    \normtwo{\Nr \cdot \vone - \diag{\mArx\ctrans[k]\mW}}^2 \leq \sigma_{\mathrm{rx}}^2 \cdot \Nr^2 \cdot \Mrx \ \forall \ k
\end{align}
%Note that magnitude of $\gtx(\thetatx^{(i)}, k)$ and $\grx(\thetarx^{(i)}, k)$ are represented at the $(i,i)$-th element of $\mAtx\ctrans[k]\mF$ and the $(j,j)$-th entry of $\mArx\ctrans[k]\mW$. 
We now draw up an optimization problem to construct an analog beamforming codebook design by aggregating the constraints and \eqref{inrrxavg}. This resulting optimization is formulated as
\begin{subequations} \label{opt1}
\begin{align}
\min_{\mF, \mW} &\quad \sum_{k=1}^{K}\normfro{\mW^*\mfH[k]\mF}^2 \label{opt1_obj1} \\
\subjectto&\quad \normtwo{\Nt \cdot \vone - \diag{\mA_{\mathrm{tx}}\ctrans[k]\mF}}^2 \leq \sigma_{\mathrm{tx}}^2 \cdot \Nt^2 \cdot \Mtx \ \forall \  k \label{opt1_const1}\\
&\quad\normtwo{\Nr \cdot \vone - \diag{\mA_{\mathrm{rx}}\ctrans[k]\mW}}^2 \leq \sigma_{\mathrm{rx}}^2 \cdot \Nr^2 \cdot \Mrx \ \forall \ k \label{opt1_const2}\\
&\quad[\mF]_{:,i} \in \mathcal{F} \ \forall \  i=1,\ldots,\Mtx \label{opt1_const3}\\
&\quad[\mW]_{:,j} \in \mathcal{W} \ \forall \ j=1,\ldots,\Mrx. \label{opt1_const4}
\end{align}
\end{subequations}

\subsection{Solution for Codebook Design}
We will set strategy in this part to solve the proposed design problem \eqref{opt1}. 
Since the discrete nature of \eqref{opt1_const3} and \eqref{opt1_const4} imposes non-convexity to the problem, we will relax this condition by expanding $\mathcal{F}$ and $\mathcal{W}$ to the continuous complex domain.
After resolving the optimization, we will project the solutions to the closest elements of $\mathcal{F}$ and $\mathcal{W}$, respectively.
Also, as the joint optimization for $\mF$ and $\mW$ incurs intractable complexity, we will mitigate this hindrance with an approximate approach, which alternatively solves the problem.
Let $\Pi_{\mathcal{F}} \big( [\mF]_{:,i} \big)$ represent the projection of the $i$-th beam collection of matrix $\mF$ onto the set of physically feasible beamforming vectors $\mathcal{F}$.
By iteratively and column-wisely applying this mapping to the $\mF$, we can expand the projection onto each column in $\mF$ as $\Pi_{\mathcal{F}}(\mF)$.
Analogously, the projection of matrix $\mW$ onto $\mathcal{W}$ is defined in the same manner.
Considering the quantized feature of $\mathcal{F}$, the $(m,n)$-th element of the projected beamforming vector can be described as
\begin{align} \label{proj_rule}
    [\Pi_{\mathcal{F}}(\mF)]_{m,n} = A\opt \cdot \exp(j \cdot \theta\opt),
\end{align}
\begin{theorem}
    The projected phase $\theta\opt$ and amplitude $A\opt$ of $[\mF]_{m,n}$ can be calculated as
    \begin{align}
        &\theta\opt = \argmin_{\theta_i \in \mathcal{P}} \ \bars{\exp(\j \cdot \theta_i) - \exp(\j \cdot \theta)}, \label{opt_theta}\\
        &A\opt = \argmin_{A_i \in \mathcal{A}} \ \bars{A_i - \cos(\theta_i - \theta^*) \cdot A}. \label{opt_A}
    \end{align}
\end{theorem}
\begin{proof}
    In a polar coordinate, the projection rule should select $(A^*, \theta^*)$, which has the shortest distance to $(A, \theta)$. The distance $d$ between the two points can be calculated as follows.
    \begin{subequations}
        \begin{align}
            d &= (A_i \cos\theta_i - A \cos\theta)^2 + (A_i \sin\theta_i - A \sin\theta)^2 \\
            &= A_i^2 + A^2 - 2A_i A \cos(\theta_i - \theta) \\
            &= (\Delta A)^2 + 4A_iA\sin^2\frac{\Delta \theta}{2}
    \end{align}
    \end{subequations}
    where $\Delta A = A_i - A$ and $\Delta \theta = \theta_i - \theta$. Therefore, $\theta\opt$ can be selected as follows.
    \begin{subequations}
        \begin{align}
            \theta\opt &= \argmin_{\theta_i \in \mathcal{P}} \ d \\
            &= \argmin_{\theta_i \in \mathcal{P}} \ (\Delta A)^2 + 4A_iA\sin^2\frac{\Delta \theta}{2} \\
            &= \argmin_{\theta_i \in \mathcal{P}} \ \bars{\exp(\j \cdot \theta_i) - \exp(\j \cdot \theta)}\label{proj_theta3}
        \end{align}
    \end{subequations}
    where \eqref{proj_theta3} comes from the fact that $\Delta A, A_i, A$ are constant. Once the $\theta\opt$ is fixed, we could select the closest amplitude, $A\opt$.
    \begin{subequations}
        \begin{align}
            A\opt &= \argmin_{A_i \in \mathcal{A}}\ d \\
            &= \argmin_{A_i \in \mathcal{A}}\ (A_i - A\cos(\Delta \theta))^2 + A^2 \sin^2(\Delta \theta) \\
            &= \argmin_{A_i \in \mathcal{A}}\ \bars{A_i - A\cos(\Delta \theta)}
        \end{align}
    \end{subequations}
\end{proof}
To approximately solve \eqref{opt1}, we initialize each codebook as $\mF \leftarrow \Pi_{\mathcal{F}} (\mAtx)$ and $\mW \leftarrow \Pi_{\mathcal{W}} (\mArx)$, both of which achieve nearly maximum gains in $\mathcal{\Atx}$ and $\mathcal{\Arx}$, respectively.
We then decompose \eqref{opt1} into two subproblems, each formulated as an optimization problem with respect to $\mF$ and $\mW$ in order to reduce the complexity of joint optimization.
With fixed $\mW$, we will convert the sum of multiple Frobenius norms in \eqref{opt1_obj1} to a single Frobenius norm, as dealing with multiple Frobenius norms can cause numerical issues.
\begin{theorem}
    \begin{align}
        \sum_{k=1}^{K}\normfro{\mW^*\mfH[k]\mF}^2 &= \normfro{\mLambda^{\frac{1}{2}}_{\mW} \mQ^*_{\mW} \mF}^2 \label{alt_obj1}
    \end{align}
\end{theorem}
where $\mLambda_{\mW}$ and $\mQ_{\mW}$ are the eigenvalue diagonal matrix and eigenvector of $ \sum_{k=1}^{K}\mfH^*[k] \mW \mW^* \mfH[k]$.
\begin{proof}
\begin{subequations}
    \begin{align} \label{opt2}
    \sum_{k=1}^{K}\normfro{\mW^*\mfH[k]\mF}^2 &\eqa \sum_{k=1}^K\trace{\mF^* \mfH^*[k] \mW \mW^* \mfH[k] \mF} \\
    &\eqb \trace{\mF^* \parens{\sum_{k=1}^{K}\mfH^*[k] \mW \mW^* \mfH[k]} \mF}\\ 
    &\eqc \trace{\mF^* \mQ_{\mW} \mLambda_{\mW} \mQ^*_{\mW} \mF} \\
    &\eqd \trace{\mF^* \mQ_{\mW} \mLambda^{* \frac{1}{2}}_{\mW} \mLambda^{\frac{1}{2}}_{\mW} \mQ^*_{\mW} \mF} \\
    &\eqe \normfro{\mLambda^{\frac{1}{2}}_{\mW} \mQ^*_{\mW} \mF}^2
\end{align}
\end{subequations}
where (a) follows from the definition of the Frobenius norm; (b) is from $\mX^* \mA \mX + \mX^* \mB \mX = \mX^* \parens{\mA + \mB} \mX$. (c) is by taking the eigenvalue decomposition $\sum_{k=1}^{K}\mfH^*[k] \mW \mW^* \mfH[k] = \mQ_{\mW} \mLambda_{\mW} \mQ^*_{\mW}$. (d) is by all of the eigenvalues are positive because for all $k$, $\mfH^*[k] \mW \mW^* \mfH[k]$ is positive semi-definite matrix.
\end{proof}
Since the discrete feature of \eqref{opt1_const3} causes non-convexity, we will relax this condition by expanding the $\mF$ to the continuous region.
Then the subproblem with fixed $\mW$ can be formulated as follows.
\begin{subequations} \label{opt3}
\begin{align}
\min_{\mF} &\quad \normfro{\mLambda^{\frac{1}{2}}_{\mW} \mQ^*_{\mW} \mF}^2 \label{obj3} \\
\subjectto&\quad \normtwo{\Nt \cdot \vone - \diag{\mA\ctrans_{\mathrm{tx}}[k]\mF}}^2 \leq \sigma_{\mathrm{tx}}^2 \cdot \Nt^2 \cdot \Mtx \ \forall \  k \label{opt3_const1}\\
&\quad \bars{[\mF]_{i,j}} \leq 1 \ \forall \  i =1,\ldots,\Nt,\ j=1,\ldots,\Mtx \label{opt3_const2}
\end{align}
\end{subequations}
After solving convex problem \eqref{opt3} with convex optimization solvers [cvx ref], we project the solution $\mF\opt$ onto the set $\sF$ as $\mF \leftarrow \Pi_{\sF}(\mF\opt)$ for feasibility. With the projected $\mF$, we can analogously reformulate \eqref{opt1_obj1} using the cyclic property of the trace : $\trace{\mA\mB\mC} = \trace{\mB\mC\mA} = \trace{\mC\mA\mB}$.
\begin{subequations}
\begin{align}
    \sum_{k=1}^{K}\normfro{\mW^*\mfH[k]\mF}^2 &= \sum_{k=1}^K \trace{\mF^*\mfH[k]\mW\mW^*\mfH\ctrans[k]\mF} \\
    &= \sum_{k=1}^K \trace{\mW^*\mfH[k]\mF\mF^*\mfH\ctrans[k]\mW} \\
    &= \normfro{\mLambda^{\frac{1}{2}}_{\mF} \mQ^*_{\mF} \mW}^2
\end{align}
\end{subequations}
We then construct the optimization problem for receiving codebook $\mW$.
\begin{subequations} \label{opt4}
\begin{align}
\min_{\mW} \ & \normfro{\mLambda^{\frac{1}{2}}_{\mF} \mQ^*_{\mF} \mW}^2 \label{opt4_obj1} \\
\subjectto
& \normtwo{\Nt \cdot \vone - \diag{\mA\ctrans_{\mathrm{rx}}[k]\mW}}^2 \leq \sigma_{\mathrm{rx}}^2 \Nr^2 \Mrx \ \forall \  k \label{opt4_const1}\\
& [\mW]_{i,j} \leq 1 \ \forall \ i=1,\ldots,\Nr,\ j=1,\ldots,\Mrx \label{opt4_const2}
\end{align}
\end{subequations}
Similar to projecting $\mF$, the solution of \eqref{opt4} is projected onto $\sW$ as $\mW \leftarrow \Pi_{\sW}(\mW\opt)$.

To represent the performance of the system, we introduce normalized sum spectral efficiency
\begin{align}
    \gamma_{\mathrm{sum}}[k] = \frac{R_{\mathrm{tx}}[k] + R_{\mathrm{rx}}[k]}{\Ctx^{\mathrm{cb}} + \Crx^{\mathrm{cb}}},
\end{align}
where $\Ctx^{\mathrm{cb}} = \log_2\parens{1+\snrtx^{\mathrm{CBF}}}$ and $\Crx^{\mathrm{cb}} = \log_2\parens{1+\snrrx^{\mathrm{CBF}}}$. $\snrtx^{\mathrm{CBF}}$ and $\snrrx^{\mathrm{CBF}}$ are maximum SNRs delivered to a given downlink-uplink user pair when $\vf_i = \Pi_{\sF}\parens{\vatx\parens{\thetatx\idx{i}}}$ and $\vw_j = \Pi_{\sW}\parens{\varx\parens{\thetarx\idx{j}}}$.

% sigmatx^2 = sigmarx^2
% 500MHz : -19dB
% 1GHz : -18dB
% 2GHz : -15.5dB
% 4GHz : -12dB
% LoneSTAR : -22dB

==> sec-keywords.tex <==
\begin{IEEEkeywords}
Full-duplex, beamforming, self-interference, phased arrays, millimeter wave.
\end{IEEEkeywords}

==> sec-peer-review-title.tex <==
% For peer review papers, you can put extra information on the cover
% page as needed:
% \ifCLASSOPTIONpeerreview
% \begin{center} \bfseries EDICS Category: 3-BBND \end{center}
% \fi
%
% For peerreview papers, this IEEEtran command inserts a page break and
% creates the second title. It will be ignored for other modes.
\IEEEpeerreviewmaketitle
